Search for VHE $\gamma$-ray emission from the globular cluster M13 with the MAGIC telescope

Based on MAGIC observations from June and July 2007, we have obtained an integral upper limit to the VHE energy emission of the globular cluster M13 of $F(E>200 \textrm{GeV})<5.1\times10^{-12} \textrm{cm}^{-2} \textrm{s}^{-1}$, and differential upper limits for $E>140 \textrm{GeV}$. Those limits allow us to constrain the population of millisecond pulsars within M13 and to test models for acceleration of leptons inside their magnetospheres and surrounding. We conclude that in M13 either millisecond pulsars are fewer than expected or they accelerate leptons less efficiently than predicted.

==> authors_last_ApJ.tex <==
% authors 16.03.2009  Format ApJ
%
\author{
H.~Anderhub\altaffilmark{a},
L.~A.~Antonelli\altaffilmark{b},
P.~Antoranz\altaffilmark{c},
M.~Backes\altaffilmark{d},
C.~Baixeras\altaffilmark{e},
S.~Balestra\altaffilmark{c},
J.~A.~Barrio\altaffilmark{c},
D.~Bastieri\altaffilmark{f},
J.~Becerra Gonz\'alez\altaffilmark{g},
J.~K.~Becker\altaffilmark{d},
W.~Bednarek\altaffilmark{h},
K.~Berger\altaffilmark{h},
E.~Bernardini\altaffilmark{i},
A.~Biland\altaffilmark{a},
R.~K.~Bock\altaffilmark{j,}\altaffilmark{f},
G.~Bonnoli\altaffilmark{k},
P.~Bordas\altaffilmark{l},
D.~Borla Tridon\altaffilmark{j},
V.~Bosch-Ramon\altaffilmark{l},
D.~Bose\altaffilmark{c},
I.~Braun\altaffilmark{a},
T.~Bretz\altaffilmark{m},
I.~Britvitch\altaffilmark{a},
M.~Camara\altaffilmark{c},
E.~Carmona\altaffilmark{j},
S.~Commichau\altaffilmark{a},
J.~L.~Contreras\altaffilmark{c},
J.~Cortina\altaffilmark{n},
M.~T.~Costado\altaffilmark{g,}\altaffilmark{o},
S.~Covino\altaffilmark{b},
V.~Curtef\altaffilmark{d},
F.~Dazzi\altaffilmark{p,}\altaffilmark{***},
A.~De Angelis\altaffilmark{p},
E.~De Cea del Pozo\altaffilmark{q},
R.~de los Reyes\altaffilmark{c},
B.~De Lotto\altaffilmark{p},
M.~De Maria\altaffilmark{p},
F.~De Sabata\altaffilmark{p},
C.~Delgado Mendez\altaffilmark{g,}\altaffilmark{*},
A.~Dominguez\altaffilmark{r},
D.~Dorner\altaffilmark{a},
M.~Doro\altaffilmark{f},
D.~Elsaesser\altaffilmark{m},
M.~Errando\altaffilmark{n},
D.~Ferenc\altaffilmark{s},
E.~Fern\'andez\altaffilmark{n},
R.~Firpo\altaffilmark{n},
M.~V.~Fonseca\altaffilmark{c},
L.~Font\altaffilmark{e},
N.~Galante\altaffilmark{j},
R.~J.~Garc\'{\i}a L\'opez\altaffilmark{g,}\altaffilmark{o},
M.~Garczarczyk\altaffilmark{n},
M.~Gaug\altaffilmark{g},
F.~Goebel\altaffilmark{j,}\altaffilmark{****},
D.~Hadasch\altaffilmark{e},
M.~Hayashida\altaffilmark{j},
A.~Herrero\altaffilmark{g,}\altaffilmark{o},
D.~Hildebrand\altaffilmark{a},
D.~H\"ohne-M\"onch\altaffilmark{m},
J.~Hose\altaffilmark{j},
C.~C.~Hsu\altaffilmark{j},
T.~Jogler\altaffilmark{j},
D.~Kranich\altaffilmark{a},
A.~La Barbera\altaffilmark{b},
A.~Laille\altaffilmark{s},
E.~Leonardo\altaffilmark{k},
E.~Lindfors\altaffilmark{t},
S.~Lombardi\altaffilmark{f},
F.~Longo\altaffilmark{p},
M.~L\'opez\altaffilmark{f},
E.~Lorenz\altaffilmark{a,}\altaffilmark{j},
P.~Majumdar\altaffilmark{i},
G.~Maneva\altaffilmark{u},
N.~Mankuzhiyil\altaffilmark{p},
K.~Mannheim\altaffilmark{m},
L.~Maraschi\altaffilmark{b},
M.~Mariotti\altaffilmark{f},
M.~Mart\'{\i}nez\altaffilmark{n},
D.~Mazin\altaffilmark{n},
M.~Meucci\altaffilmark{k},
M.~Meyer\altaffilmark{m},
J.~M.~Miranda\altaffilmark{c},
R.~Mirzoyan\altaffilmark{j},
H.~Miyamoto\altaffilmark{j},
J.~Mold\'on\altaffilmark{l},
M.~Moles\altaffilmark{r},
A.~Moralejo\altaffilmark{n},
D.~Nieto\altaffilmark{c},
K.~Nilsson\altaffilmark{t},
J.~Ninkovic\altaffilmark{j},
N.~Otte\altaffilmark{j,}\altaffilmark{**},
I.~Oya\altaffilmark{c},
R.~Paoletti\altaffilmark{k},
J.~M.~Paredes\altaffilmark{l},
M.~Pasanen\altaffilmark{t},
D.~Pascoli\altaffilmark{f},
F.~Pauss\altaffilmark{a},
R.~G.~Pegna\altaffilmark{k},
M.~A.~Perez-Torres\altaffilmark{r},
M.~Persic\altaffilmark{p,}\altaffilmark{v},
L.~Peruzzo\altaffilmark{f},
F.~Prada\altaffilmark{r},
E.~Prandini\altaffilmark{f},
N.~Puchades\altaffilmark{n},
I.~Reichardt\altaffilmark{n},
W.~Rhode\altaffilmark{d},
M.~Rib\'o\altaffilmark{l},
J.~Rico\altaffilmark{w,}\altaffilmark{n},
M.~Rissi\altaffilmark{a},
A.~Robert\altaffilmark{e},
S.~R\"ugamer\altaffilmark{m},
A.~Saggion\altaffilmark{f},
T.~Y.~Saito\altaffilmark{j},
M.~Salvati\altaffilmark{b},
M.~Sanchez-Conde\altaffilmark{r},
K.~Satalecka\altaffilmark{i},
V.~Scalzotto\altaffilmark{f},
V.~Scapin\altaffilmark{p},
T.~Schweizer\altaffilmark{j},
M.~Shayduk\altaffilmark{j},
S.~N.~Shore\altaffilmark{x},
N.~Sidro\altaffilmark{n},
A.~Sierpowska-Bartosik\altaffilmark{q},
A.~Sillanp\"a\"a\altaffilmark{t},
J.~Sitarek\altaffilmark{j,}\altaffilmark{h},
D.~Sobczynska\altaffilmark{h},
F.~Spanier\altaffilmark{m},
A.~Stamerra\altaffilmark{k},
L.~S.~Stark\altaffilmark{a},
L.~Takalo\altaffilmark{t},
F.~Tavecchio\altaffilmark{b},
P.~Temnikov\altaffilmark{u},
D.~Tescaro\altaffilmark{n},
M.~Teshima\altaffilmark{j},
M.~Tluczykont\altaffilmark{i},
D.~F.~Torres\altaffilmark{w,}\altaffilmark{q},
N.~Turini\altaffilmark{k},
H.~Vankov\altaffilmark{u},
R.~M.~Wagner\altaffilmark{j},
W.~Wittek\altaffilmark{j},
V.~Zabalza\altaffilmark{l},
F.~Zandanel\altaffilmark{r},
R.~Zanin\altaffilmark{n},
J.~Zapatero\altaffilmark{e},
}
\altaffiltext{a} {ETH Zurich, CH-8093 Switzerland}
\altaffiltext{b} {INAF National Institute for Astrophysics, I-00136 Rome, Italy}
\altaffiltext{c} {Universidad Complutense, E-28040 Madrid, Spain}
\altaffiltext{d} {Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}
\altaffiltext{e} {Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}
\altaffiltext{f} {Universit\`a di Padova and INFN, I-35131 Padova, Italy}
\altaffiltext{g} {Inst. de Astrof\'{\i}sica de Canarias, E-38200 La Laguna, Tenerife, Spain}
\altaffiltext{h} {University of \L\'od\'z, PL-90236 Lodz, Poland}
\altaffiltext{i} {Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}
\altaffiltext{j} {Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}
\altaffiltext{k} {Universit\`a  di Siena, and INFN Pisa, I-53100 Siena, Italy}
\altaffiltext{l} {Universitat de Barcelona (ICC/IEEC), E-08028 Barcelona, Spain}
\altaffiltext{m} {Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany}
\altaffiltext{n} {IFAE, Edifici Cn., Campus UAB, E-08193 Bellaterra, Spain}
\altaffiltext{o} {Depto. de Astrofisica, Universidad, E-38206 La Laguna, Tenerife, Spain}
\altaffiltext{p} {Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}
\altaffiltext{q} {Institut de Cienci\`es de l'Espai (IEEC-CSIC), E-08193 Bellaterra, Spain}
\altaffiltext{r} {Inst. de Astrof\'{\i}sica de Andalucia (CSIC), E-18080 Granada, Spain}
\altaffiltext{s} {University of California, Davis, CA-95616-8677, USA}
\altaffiltext{t} {Tuorla Observatory, University of Turku, FI-21500 Piikki\"o, Finland}
\altaffiltext{u} {Inst. for Nucl. Research and Nucl. Energy, BG-1784 Sofia, Bulgaria}
\altaffiltext{v} {INAF/Osservatorio Astronomico and INFN, I-34143 Trieste, Italy}
\altaffiltext{w} {ICREA, E-08010 Barcelona, Spain}
\altaffiltext{x} {Universit\`a  di Pisa, and INFN Pisa, I-56126 Pisa, Italy}
\altaffiltext{*} {now at: Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), E-28040 Madrid, Spain}
\altaffiltext{**} {now at: University of California, Santa Cruz, CA 95064, USA}
\altaffiltext{***} {supported by INFN Padova}
\altaffiltext{****} {deceased}


